Counterexample-Driven Synthesis for Probabilistic Program Sketches

Probabilistic programs are key to deal with uncertainty in e.g. controller synthesis. They are typically small but intricate. Their development is complex and error prone requiring quantitative reasoning over a myriad of alternative designs. To mitigate this complexity, we adopt counterexample-guided inductive synthesis (CEGIS) to automatically synthesise finite-state probabilistic programs. Our approach leverages efficient model checking, modern SMT solving, and counterexample generation at program level. Experiments on practically relevant case studies show that design spaces with millions of candidate designs can be fully explored using a few thousand verification queries.

==> 02-problem.tex <==

\section{Problem Formulation}

We first describe the elementary elements of our synthesis problem: 
1)~modelling the design space of a system under design, and  
2)~specifying non-functional quantitative properties, 
%and 3)~the notation of counter-examples providing the evidence that the candidate design 
%violates a property. 
and then formulate two (related) program synthesis problems.  

\subsection{Design space modelling\label{sec:designSpaceModelling}}
Probabilistic systems are typically specified by means of a high-level modelling language, such as PRISM~\cite{KNP11}, JANI~\cite{JANI} or MODEST~\cite{MODEST}.  
We propose a \emph{sketching language} based on the PRISM guarded-command language~\cite{KNP11} that allows us to succinctly define the design space. 
We start off by briefly describing a subset of the PRISM language whose programs yield a \emph{Discrete-Time Markov Chain} (DTMC).

\begin{mydef}[DTMC]	
A DTMC is a triple $(S,\mathbf{P}, \init)$, where $S$ is a finite set of states, $\mathbf{P}: S \times S \rightarrow [0,1]$ is a transition probability matrix, and $\init \in S$ is an initial state. 
State $s$ is a \emph{deadlock} if $\sum_{s' \in S} \mathbf{P}(s,s') = 0$.
The operation $\fixdeadlock$ sets $\mathbf{P}(s,s') = 1$ for each deadlock $s$.
\end{mydef}

A PRISM program is a parallel composition of a finite set of modules. 
Although our synthesis approach works for each PRISM program, for the sake of simplicity, we consider programs consisting of a single module in our presentation.
This is not a restriction as every PRISM program can be flattened into single-module form.
%\footnote{By means of a syntactic transformation in which the guards of synchronising commands are conjuncted while multiplying the probabilities of the individual updates.}.
A program has a finite set $\Vars$ of bounded integer variables.
Let $\Assignments{\Vars}$ denote the set of all variable assignments, i.e., functions $s \colon \Vars\to\mathbb{Z}$ with $s(\var)\in\dom(\var)$ for all $\var\in\Vars$.  
Variable assignments define program states.
A program contains \emph{commands} of the form
%%
 \begin{align} 
   c \ = \ g\to\ p_1: f_1 + \ldots + p_n: f_n
  \end{align}
%%
where 
$g \in \Assignments{\Vars} \to \{ 0, 1 \}$ is a Boolean predicate (``guard'') over the variables in $\Vars$, $p_j \in [0,1]$ is an expression $\Assignments{\Vars} \rightarrow [0,1]$ with $\forall s \in \Assignments{\Vars}$, $\sum_{j=1}^n p_j(s) = 1$, and $f_j\colon \Assignments{\Vars}\to\Assignments{\Vars}$ is a variable-update function.
A command with guard $g$ is \emph{enabled} in a variable assignment $s \in \Assignments{\Vars}$, if $g(s) = 1$.   
The set  $\enabled(s)$ denotes commands enabled in state $s$.
% if it is empty, $s$ is a deadlock.
Executing an enabled command results in update $f_j$ with probability $p_j$.

%\color{red}
%[ToDo When and how to speak about the multi-module programs]
%
%To avoid a complicated notation, we will further assume that there is only one module and no synchronisation. Note that every PRISM program 
%can be translated into this form (so called flatting). All modules comprising commands with the same synchronisation action have to synchronise (i.e., to carry out one of these commands simultaneously) and the resulting probability of such synchronised commands is equal to the multiplication of the individual update probabilities. 
%\color{black}

\begin{mydef}[Program]
A \emph{(PRISM) program} $\mathfrak{P}$ is a pair of bounded integer variables and (finitely many) commands $(\Vars, C)$, where each command $c \in C$ is a triple $(g, p, f)$. 
Its semantics $\semantics{\mathfrak{P}}$ is the DTMC $(\Assignments{\Vars}, \mathbf{P}, s_0)$.
For $s, s'\in \Assignments{\Vars}$ with $\enabled(s) \neq \emptyset$, the transition matrix $\mathbf{P}$ is defined~as
\[ 
\mathbf{P}(s,s') = \frac{\Big(\sum_{c \in \enabled(s)} \sum_{i} [f_i(s) = s'] \cdot p_i\Big)}{|\enabled(s)|}, 
\] 
where $[f_i(s) = s']$ is the indicator function which returns $1$ if the update $f_i$ yields $s'$ and 0 otherwise. 
The initial state $\init$ is given by the initial variable assignment given in $\mathfrak{P}$.
\end{mydef}

A program $\mathfrak{P}$ is \emph{non-overlapping} if $|\enabled(s)| \leq 1$ for each state $s$ reachable from $\mathfrak{P}$'s initial state $\init$.

%The state of a module is encoded by a set of 
%finite-range local variables, and its state transitions are defined by probabilistic 
%guarded commands that change these variables, and have the general form:
%	
%	\begin{small}
%		\begin{equation}
%		\begin{array}{l}
%		\textsf{ [action] guard } \rightarrow e_1 : update_1 + \ldots +  e_n : update_n
%		\end{array}
%		\label{eq:lan}
%		\end{equation}
%		\vspace{-1em}
%	\end{small}
%	
%	
%In this command, \emph{guard} is a Boolean expression over all model variables. 
%If the guard evaluates to \textsf{true}, the arithmetic expression $e_i$, $1 \leq i \leq n$, 
%	gives the probability with which the \emph{update}$_i$ change of the module variables occurs. 
%When \emph{action} is present, all modules comprising commands with this action have to synchronise (i.e., to carry out one of these commands simultaneously) and the resulting probability of such synchronised commands is 
%\color{blue} equal to the multiplication of the individual update probabilities. 
%In the presence of synchronisations, a program is non-overlapping, if the corresponding one-module symbolic description is non-overlapping.
%	
%	
%	\color{red}
%	 [.. I suggest to replace the example with a motivating paragraph with a code snippet ..]
%	 [Fine with me]
%	 \color{black}
	 
%	 Before providing the formal definition of our sketching language, we will motivate the particular sketching constructs we use. 
%	 \emph{Program constants:} 
%	 Typical PRISM program contains several constants/parameters affecting the structure and dynamic of the underlying DTMC, and thus various quantitative attributes designers are interested in. As example, we could consider a size of the buffer in a producer-consumer problem. 
%	  \color{red}[ToDo]. \emph{Guards} [ToDo]. 
%	 \emph{Effects} [ToDo]. 
%	 
	 
%\lstset{language=Prism}   
%\newsavebox{\buffer}
%\begin{lrbox}{\buffer}% Store first listing
%\begin{lstlisting}
%hole H1 either { 5..10 }
%hole H2 either { 0, 1, 2 }
%relation R either { <=, =, >=}
%variable V either { size, state}
%operation O either {-,+}
%const int capacity = H1;
%module buffer
%size : [0..size] init 0;
%state : [0..2] init 2;
%...
%[]  s=H2 & size R capacity/2 -> 1: V = size O 1;
%\end{lstlisting}
%\end{lrbox}

%\begin{figure}
%\scalebox{0.92}{\usebox{\buffer}}
%\caption{Sketching example. \color{red} [ToDo Fix the example]}
%\label{fig:sketch}
%\end{figure}	 
	
Briefly speaking, a (PRISM) sketch is a program that may contain ``\emph{holes}''.
Holes are the unknown parts of the program and can be replaced by one of finitely many \emph{options}.
%% 
\begin{mydef}[Program hole]
A \emph{hole} $h$ is of the form: 
\begin{align}
  \texttt{hole $h$ either $\{$ $e_1, \hdots, e_n$ $\}$}
\end{align}
where $h$ is the hole identifier and $e_i$ is a program expression over the variables in $\Vars$.
Let $\Option_h = \{$ $e_1, \hdots, e_n$ $\}$, the options with which hole $h$ can be replaced, and $\Option_H$ denote the point-wise lifting to the set $H$ of holes.
\end{mydef}

A hole $h$ can be used in commands in a similar way as a constant, and may occur multiple times within a command. 
%If all possible values of $h$ are variables, a state may map a variable onto hole $h$.
To facilitate the formulation of restrictions, options can be named:
\begin{align}
  \texttt{hole $h$ either $\{ x_1 \text{ is } e_1 \text{ price } c_1, \hdots \, \}$} \label{eqn:general_hole_definition}
\end{align}
where option $e_1$ is named $x_1$, etc.
Propositional formulae over option names restrict hole instantiations, e.g., 
\begin{align}
  \texttt{constraint $(x_1 \lor x_2) \implies x_3$ }
\end{align}
requires that whenever the options $x_1$ or $x_2$ are taken for some (potentially different) holes, option $x_3$ (of a third hole) is also taken.
To distinguish cheap and expensive options, \eqref{eqn:general_hole_definition} allows a hole to have a non-negative integer price (or cost).
By default, the price is zero and default prices are typically omitted.
%% We leave the design of concise patterns as shorthands for the more elaborate formulae as future work.

As stated above, holes represent expressions.
To further ease specifying the design space, we add some other types of holes:
\begin{align}
  & \texttt{relation $r$ either $\{ r_1, \hdots, r_n \}$} \\
  & \texttt{operation $o$ either $\{ o_1, \hdots, o_n \}$} \\
  & \texttt{variable $v$ either $\{ v_1, \hdots, v_n\}$} 
%& \texttt{assignment NAME either $\{ a_1, \hdots, a_k \}$}
\end{align}
 They can be encoded in terms of expression holes as in \eqref{eqn:general_hole_definition}.
 % and are thus syntactic sugar.
%%	
\begin{mydef}[Program sketch]
A \emph{(PRISM) program sketch} is a pair $\Sketch = (\mathfrak{P}_H, \Option_H)$ where $\mathfrak{P}_H$ is a program with a set $H$ of holes with options $\Option_H$.
\end{mydef}	

\lstset{language=Prism}   
\newsavebox{\sketch}
\begin{lrbox}{\sketch}% Store first listing
\begin{lstlisting}
hole X either { XA is 1 price 3, 2}
hole Y either { YA is 1, 3 }
hole Z either { 2, 3 }
constraint  !(XA && YA);
module rex
s : [0..3] init 0;
s = 0 -> 0.5: s'=X + 0.5: s'=Y;
s = 1 -> s'=Z; 
s = 2 -> s'=2;
s = 3 -> s'=3;
endmodule
\end{lstlisting}
\end{lrbox}
\newsavebox{\instance}
\begin{lrbox}{\instance}% Store first listing
\begin{lstlisting}
module rex
s : [0..3] init 0;
s = 0 -> 0.5: s'=1 + 0.5: s'=3;
s = 1 -> s'=3; 
s = 2 -> s'=2;
s = 3 -> s'=3;
endmodule
\end{lstlisting}
\end{lrbox}

\begin{figure}
\subfloat[Program sketch $\Sketch$]{\scalebox{0.85}{\usebox{\sketch}}
\label{fig:runningexample:sketch}
} \hfill%
\subfloat[Instance $\ProgHoles(\{ X{\mapsto}1, Y, Z{\mapsto}3 \})$]{\scalebox{0.92}{\usebox{\instance}}
\label{fig:runningexample:instance}
}
%\subfloat[Instance for ${ \text{X} \mapsto 1, \text{Y} \mapsto 1, \text{Z} \mapsto 3 \}$]{
%
%}
\caption{Running example}
\end{figure}

\begin{example}
\label{ex:runningex:sketch}
\label{ex:runningex:dtmcs}
We consider a small running example to illustrate the main concepts.
Fig.~\ref{fig:runningexample:sketch} depicts the program sketch $\Sketch$ with 
holes $H = \{ \text{X}, \text{Y}, \text{Z} \}$.
For \text{X}, the options are $\Option_\text{X} = \{ 1, 2 \}$.
The constraint forbids \text{XA} and \text{XB} both being one; it ensures a non-trivial random choice in state \texttt{s=0}.
\end{example}
	
%[The stuff below should be rather straightforward to realise, but actually implementing them seems the lowest priority. Just checked: artefacts only have to be submitted after paper is accepted, and as the submission is double blind, we are supposed \textbf{not} to make code public before]
%[Not sure how to introduce the syntax, do we want to do it more formally? ]	 
%
%\color{red} [ToDo Properly introduce and define the notation of the price for the option]
%
%Named options can be attached a price \texttt{$x_1$ is $e_1$ price $c_1$, ..} 
%
%
%[ToDo Which constructs we want to present?]
%
%The use of constraints also allows us extend the sketch with holes in relations, operators and assignments. 
%\begin{align}
%& \texttt{relation NAME either $\{ r_1, \hdots r_n \}$} \\
% & \texttt{operation NAME either $\{ o_1, \hdots o_n \}$} \\ 
%&  \texttt{variable NAME either $\{ v_1, \hdots, v_k\}$} 
%%& \texttt{assignment NAME either $\{ a_1, \hdots, a_k \}$}
%\end{align}
%
%
%
%%[For analysis, the extended PRISM-Sketch is reduced to the standard PRISM-Sketch, see Sect.~\ref{sec:algorithmic:extendedprism}.]
%%For relations and operations:
%%\texttt{relation NAME either $\{ r_1, \hdots r_n \}$} and \texttt{operation NAME either $\{ o_1, \hdots o_n \}$}, with $r_i$ and $o_i$ relations and operations, respectively.
%%For assignments,
%%\texttt{assignment NAME either $\{ v_1, \hdots, v_k\}$} with the variables either global or local variable names, or the reserved keyword \texttt{none}. An assigment-hole may with local variable options may only be used in a single module, and the local variable names must then be defined within this module.
%
%
%
%[ToDo Add a remark about multi-module sketches and also that the constructs (4)-(6) can be encoded use the construct~(3).]
%
%[ToDo Still not sure about this example]
%\begin{example}
%Fig.~\ref{fig:sketch} illustrates a short snippet  of a sketch describing a buffer module. The hole $H1$ is used to define the capacity of the buffer. The snippet then includes one partially specified command. The guard of the command depends on the hole $H2$ encoding the required state of the module and on the hole $R$ (of the type relation) encoding the required relationship between the current size of the buffer and its capacity. Finally, the partially specified effect of the command updates the variable given by the hole $V$ (of the type variable) using the value of the variable $size$ increased or digressed by~1, depending on the hole $O$ (of the type operation).
%\end{example}
%%\color{black}
We obtain programs by instantiation of the holes.

\begin{mydef}[Realisations]
\label{def:realisation}
For program sketch $\Sketch = (\mathfrak{P}_H, \Option_H)$, a \emph{realisation} of the set $H$ of holes is a function $r \colon H \rightarrow \Option_H$ with $\forall h \in H.~r(h) \in \Option_h$ and that satisfies all constraints in $\mathfrak{P}_H$.
%The price $\Gamma(r)$ of realisation $r$ is the sum of the 
Its price $\Gamma(r)$ is the sum of the 
prices of the options taken by $r$.
The \emph{program instance} $\ProgHoles(r)$ for realisation $r$ is the program $\mathfrak{P}_H[H / r]$ in which each hole $h \in H$ in $\mathfrak{P}_H$ is replaced by $r(h)$.
\end{mydef}
We also use $\Sketch(r)$ to denote $\ProgHoles(r)$.
Sketch $\Sketch$ can thus be regarded as describing the finite set $\{ \semantics{\ProgHoles(r)} \mid r$ is a realisation of $\Sketch \}$ of DTMCs.

\begin{example}
\label{ex:extrarealisations}
Consider our running example.
The program in Fig.~\ref{fig:runningexample:instance} depicts the instance $\Sketch(r)$ for realisation $r$ with $r(X) = 1, r(Y) = r(Z) = 3$. 
It follows that $\Gamma(r) = 3$ as the option 1 for $X$ has price three and all other selected options have cost zero.
For realisation $r' = \{ Y \mapsto 1, X, Z \mapsto 2 \}$, 
	% is depicted in Fig.~\ref{fig:runningex:dtmc2} and 
$\Gamma(r') = 0$.
The assignment $\{ X, Y \mapsto 1, Y \mapsto 3 \}$ violates the constraint and is not a realisation.
In total, $\Sketch$ represents $6 = 2^3{-}2$ DTMCs.
\end{example}

\color{black}
	
%	The formal  semantics of a sketch can be expressed by parametric DTMCs
%
%\begin{mydef} [$p$DTMC]
%	\label{def:pDTMC}
%	Let $D$ be a finite set of discrete parameters such that 
%	the domain of each parameter $d\in D$ is a finite set 
%	$T^d\!\subset\! \mathbb{Z}$. Let $q\colon D \rightarrow \mathbb{Z}$ be a realisation satisfying that $\forall d\in D:$ $q(d) \in T^d$.
%	 A $p$DTMC over $D$ is a tuple\\[-3mm]
%	\begin{equation}
%	\mathfrak{C}_D=(S_D, init_D, \mathbf{P}_D, L_D), 
%	\label{eq:pctmc}
%	\end{equation}
%	
%	\noindent
%	where, for any realisation $q$:\\
%	\squishlist
%	\item  $S_D(q) = S$ is a finite set of {\em states}, 
%	\item $init_D(q)\in S$ is the initial state;
%	\item $\mathbf{P}_D(q): S \times S  \rightarrow [0,1]$ is a {\em 
%	probability matrix},
%	%\item $\mathcal{D}_{init}(q)\in S$ is an initial state;
%	\item $L_D(q): S \rightarrow 2^{AP}$ is a {\em labelling function} mapping each state $s 
%	\in S$ to the set $L(q)(s) \subseteq AP$ of atomic propositions that hold true in $s$.
%	\squishend 
%\end{mydef}
%
%A $p$DTMC $\mathfrak{C}_D$ describes the finite set of discrete-time 
%Markov chains $\{ \mathfrak{C}_D(q) \, | \,  q \mbox{ is a realisation} \}$, where each 
%$\mathfrak{C}_D(q)  =(S_D(q), init_D(q), \mathbf{P}_D(q), L_D(q))$, 
%is the instantiated DTMC.	
%	
%		
%	The translation of  a sketch $\mathfrak{S}_H$, where each $h \in H$ has a finite number of  realisations, into the 
%	corresponding $p$DTMC $\mathfrak{C}_D$ is fully automatic and follows the probabilistic guarded command 
%	semantics described above. 
%	
%\color{blue}
%'pDTMC' is a multiset!	
%	
%\color{red}
%	
%	\begin{proposition}
%The sketch $\mathfrak{S}_H$ is a symbolic representation of the $p$DTMC $\mathfrak{C}_D$ iff there exists mappings $m_s$ and $m_d$ such that 
%\begin{itemize}
%\item for each realisation $r$ of $\mathfrak{S}_H$, $m_s(r)$ is realisation of  $\mathfrak{C}_D$ such that  $\semantics(\mathfrak{S}_H(r)) = C(m_s(r))$
%\item for each realisation $q$ of  $\mathfrak{C}_D$, $m_d(q) $ is realisation of $\mathfrak{S}_H$  such that  $C(m_d(q)) = \semantics(\mathfrak{S}_H(q))$
%\end{itemize} 
%\end{proposition}
%[Note that we probably don't want to require a bijection between  $\mathcal{R}^v_H$ a $\mathcal{Q}$.]



%I don't think we need figures for the DTMCs.
%\begin{figure}
%\subfloat[]{
%\begin{tikzpicture}
	
%\end{tikzpicture}
%\label{fig:runningex:dtmc1}
%}
%\subfloat[]{
%\begin{tikzpicture}
	
%\end{tikzpicture}
%\label{fig:runningex:dtmc2}
%}
%\caption{\color{red} [ToDo] The corresponding DTMCs for two instantiations}	
%\end{figure}

\color{black}

\subsection{Property specification language}
%\color{blue}
%[As we can only do upper bounds for rewards, I would strongly prefer to call it costs. Only specifying upper bounds for costs seems much more reasonable :-) ]
%\color{black}

To specify quantitative properties over the SUD, we use the \textit{probabilistic computation tree logic} (PCTL). 
It comprises state formulae ($\Phi$) and path formulae ($\phi$) with the syntax:
	
	\vspace*{-2.75mm}
	\begin{equation}
	\begin{array}{l}
	\Phi ::= \mathsf{true} \mid a \mid \neg\Phi \mid \Phi \wedge \Phi \mid 
	P_{\sim \lambda}[\phi]  \\
	\phi ::= X\mbox{~}\Phi \mid \Phi \ U^{\leq k} \Phi
	\end{array}\; ,
	\label{eq:csl}
	\end{equation}
	
	\vspace*{-1.7mm}
	\noindent
	where $a$ is an atomic proposition evaluated over states, ${\sim \ \in \left\{ 
		<, \leq, \geq, > \right\}}$, and $\lambda \in [0,1]$ is a
	%or reward ($r \in \mathbb{R}_{\geq 0}$) 
	threshold,
	%\footnote{For 
	%	simplicity, we use $\sim r$ to denote the threshold for both probability and 
	%	reward quality attributes.}, 
	and $k\in 
	\mathbb{N} \cup \{ \infty \}$ is a number of steps. A `future' operator, $F$, and `globally' operator, $G$, are derived in the standard way.
	
	%\footnote{$P_{\sim r}[F^{\leq k} \Phi] = 
	%	P_{\sim r}[\mathsf{true} \ U^{\leq k} \Phi]$ and $P_{\sim r}[G^{\leq k} \Phi] = 
	%	P_{\overline{\sim} 1-r}[F^{\leq k} \neg \Phi]$}. 
	
	The PCTL semantics is defined using a satisfaction relation $\vDash$; e.g., 
	$s \vDash P_{\sim \lambda}[\phi]$ iff $\Prob(s,\phi)\! \sim\! \lambda$ where  $\Prob(s,\phi)$
	denotes the probability of the set of paths (sequences of states) satisfying $\phi$ 
	that start in $s$. 
	Intuitively, a path satisfies formula $\Phi\mbox{~}U^{\leq k}\mbox{~}\Psi$ if within $k$ steps there is state satisfying $\Psi$ and all preceding states satisfy $\Phi$.
%	A path $\omega = 
%	s_0t_0s_1t_1\ldots$  satisfies the formula $\Phi\mbox{~}U^{\leq k}\mbox{~}\Psi$ iff there 
%	exists  $l \in \mathbb{N}$ such that $(  l \leq k  \wedge {\omega @ l
%	\vDash \Psi} \wedge \forall l' \leq l. \omega @ l' \vDash \Phi)$, where $\omega@l$ 
%	denotes the state in $\omega$ at discrete step~$l$.
	To simplify the notation, let $\Prob(\ProgHoles(r), \phi)$ denote the probability 	of the set of paths in the DTMC $\semantics{\ProgHoles(r)}$ that start in the initial state and satisfy $\phi$.
	Then $\ProgHoles(r) \vDash P_{\sim \lambda}[\phi]$ iff $\Prob(\semantics{\ProgHoles(r)}, \phi) \! \sim\! \lambda$.

To further support quality attributes specified using reward (or cost) properties~\cite{stochastic-model-checking1} we consider a mild extension of PCTL. 
To that end, DTMCs are equipped with a state reward ${\rho\colon S \rightarrow \mathbb{R}_{\geq 0}}$, and PCTL is extended with state formulas
		\begin{equation}
	\begin{array}{l}
	\Phi ::= R_{\sim \lambda}[F\, \Psi] \mid R_{\sim \lambda}[C^{\leq k}]  \\
	\end{array}\; ,
	\label{eq:rewd}
	\end{equation}
	where ${\sim \ \in \left\{ 
		<, \leq \right\}}$, and $\lambda \in \mathbb{R}_{\geq 0}$ is a reward threshold.
Intuitively, $s \vDash R_{\sim \lambda}[C^{\leq k}]$ if, from state $s$, the expected reward accumulated after $k$ steps satisfies ${\sim}\lambda$, and $s \vDash R_{\sim \lambda}[F\, \Psi]$ if from state $s$ the expected reward accumulated until reaching a $\Psi$-state meets ${{\sim} \lambda}$.
The satisfaction relation for states and DTMCs can be straightforwardly extended to reward properties.
%% We justify the restriction to upper bounds in reward properties in Section~\ref{sec:details:counterex}.	
	
\begin{example}
\label{ex:runningex:sat} 
Reconsider $\Sketch$, $r$, and $r'$ from Ex.~\ref{ex:extrarealisations}. 
Let $\Phi =  P_{\leq 0.4} [F~\texttt{s=3}]$. 
While $\Sketch(r) \not \vDash \Phi$, we have $\Sketch(r') \vDash \Phi$.
\end{example}
	
%\subsection{Counter-examples}
%The notation of counter-examples (CEs) that provide evidence and explanation why a non-valid candidate program violates a given specification represents the essential element of our synthesis framework. In particular, we use CEs to steer the search for the desired program and, more importantly, to prune the search space. Counter-example generation for probabilistic programs is not easy.  Showing that the reachability probability of a error state $s$ does not stay below a given threshold $\lambda$ (the simplest quantitative verification query)  requires a set of finite paths leading to $s$, whose probability mass exceeds $\lambda$. 
%
%There are two approaches for the CE generation: 1) a state level CEs~\cite{CE2009} that typically leverages a $k$-shortest path algorithm to identify the most probable paths leading to the error state $s$ and 2) a program level approach~\cite{Dehnert2014} that identifies the minimal critical subprogram (i.e. the minimal set of commands) that induces a set of paths leading to $s$ with a probability large than $\lambda$. The crucial problem of the state level approach is the size of the set of paths that can be doubly exponential in the number of states and thus not effectively usable for pruning the design space. In particular, any generalisation that would adhere to the sketch is not~feasible.
%
%Therefore, we build our framework on the program level CEs. In particular, we employ the technique of~\cite{Dehnert2014} that reduces the computation of the minimal critical subprogram to repeatedly solving \texttt{MaxSat} instances over two sets of propositional formulae, $\Phi$ and $\Psi$. The set $\Phi$ encodes selection of  a set of commands  -- via a negation the \texttt{MaxSat} solver tries to minimises the size of the command set.  The set $\Psi$ encodes a set of required (but not sufficient)  constrains on the valid CEs (initially it says e.g. that $s$ is reachable from the initial state). In this way,  the \texttt{MaxSat} solver returns a candidate $E$  (a set of commands) for the minimal CE. Using a standard verification procedure is then checked whether the candidate $E$ induces a set of path leading to $s$ with a probability larger than $\lambda$. If do so, we found the minimal CE (the minimality of $E$ is ensured by the construction). Otherwise, we extend the set $\Psi$ to rule out $E$ and other insufficient candidate command sets.  In particular, these new conditions require that the probability to reach $s$ is increased (with respect to $E$) in the new candidates. For further details, we refer to~\cite{Dehnert2014}. Note that apart from a more compact representation of CEs, the generation of program level CEs provides significantly better scalability comparing to state level approaches.
%
%[Add formal definition of the CE $E$ as a set of commands, and define the DTMC $D$ induced by $E$ (the notation of  $D_{\mid E}$)] 

\subsection{Problem formulation}
\label{sec:problem}
%\color{red} [ToDo We need to agree on which problems we want to formalise here. I suggest  two problems: 1) synthesis problem including set of a PCTL-based constrains + optionally the prize constrain and 2) optimal synthesis problem including  a set of  constrains as in 1) + one optimisation objective. The optimisation objective can be defined using probability (we support min/max), reward (we support min) a prize (we support min)] 
%\color{black}

We consider two related synthesis problems.
The first problem, simply called \emph{synthesis}, considers a sketch (in the above language), a finite set of PCTL formulas and a budget $B \in \mathbb{N}$.
A solution to this problem is a program adhering to the sketch, the PCTL formulas and the budget.
If such a solution does not exist, the synthesis algorithm shall return $\texttt{Unsat}$.

Let realisation $r$ of sketch $\Sketch$ be $(B, \{\Phi_{i}\}_{i\in I})$-\emph{feasible} for budget $B$ and PCTL formulas $\{\Phi_{i}\}_{i\in I}$ whenever its cost is within the budget while fulfilling all PCTL properties, i.e., $\Gamma(r) \leq B$ and $\Sketch(r) \vDash \Phi_i$, for all $i \in I$.

\begin{problem}[Synthesis]
\label{prob:syn}
Let $\{\Phi_{i}\}_{i\in I}$ be a finite set of PCTL state-formulas, $\Sketch$ a program sketch, and $B \in \mathbb{N}$ a budget.
The \emph{synthesis problem} is to find any $(B, \{\Phi_{i}\}_{i\in I})$-feasible realisation $r$ of $\Sketch$, or report that no such $r$ exists.
\end{problem}

The second problem, called \emph{optimal synthesis}, is motivated by engineering problems where a set of hard constraints on the system is supplemented by an optimisation objective.
In our case, this objective can refer to either the satisfaction probability of a certain PCTL path formula, expected rewards or the realisation's price.
For simplicity, we formalise the optimal synthesis problem for a minimal probability objective.
Other objectives and multiple objectives can be defined analogously. 

%In many engineering problems, designers are not only interested in systems satisfying a set of quantitative constrains (e.g. in the synthesis of a system satisfying having the probability of a failure below 1\% and the expected energy consumption below 10kJ), but they have to solve more complicated synthesis problems including an optimisation of certain quantitative objective (e.g. find a system with the probability of a failure below 1\% having the minimal expected energy consumption). This type of problems can be formalise as the \emph{optimal synthesis}. We show that our synthesis framework is capable to solve these problems as it can effectively prove that there is no system having the required failure rate and having the expected energy consumption below a certain threshold. Note that, the following synthesis problem can be extended to multiple optimisation objectives and approximate it by multiple single objective optimisation  queries.     

%\color{blue}
%[... Maybe it is good to have phi contain two properties here, which would be more interesting for the verifier part, but annoying for the synthesiser part]
%\color{black}

\begin{problem}[Optimal synthesis] 
\label{prob:opt}
Let $\{\Phi_{i}\}_{i\in I}$ be a finite set of PCTL formulas, $\Sketch$ be a program sketch, and $B \in \mathbb{N}$ a budget. 
For $\epsilon \in \mathbb{Q} \cap (0,1]$ and PCTL path-formula $\phi$, the \emph{$\epsilon$-optimal synthesis} problem is to find any $(B, \{\Phi_{i}\}_{i\in I})$-feasible realisation $r$ of $\Sketch$ such that for all $(B, \{\Phi_{i}\}_{i\in I})$-feasible realisations $r'$ of $\Sketch$, it is $\epsilon \cdot \Prob(\Sketch(r), \phi) \leq \Prob(\Sketch(r'), \phi)$, or report that no such $r$ exists.
\end{problem}

The accuracy factor $\epsilon$ allows us to control the relative accuracy of the found optimum.
For instance, $\epsilon = 0.95$ seeks solutions whose probability is minimal up to $5\%$.
% We discuss in Section~\ref{sec:discussion} how our framework can handle such synthesis problems.   

%\color{blue}
%[I would leave the multi-objective for the discussion/future work section]
%We will address the optimisation problem by adequately adapting the synthesis loop which solves Problem~\ref{prob:syn}, where we iteratively searc
%The generation of a Pareto-front for multiple optimisation objectives is then a straightforward generalisation, in which we prune any non-Pareto 
%. In that case we would be interested in computing the Pareto front of the solutions. Although this problem can be approximated by multiple single objective optimisation  queries and thus effectively solved by our approach, we leave this direction to future work.

%\color{red} [Should we add an example -- it seems we starting to have too many examples??] \color{black}



%The maximal synthesis problem can be defined a similar way. Also note that we support optimisation objectives in the form of the minimisation of a reachability or cumulative  reward presented in the previous section as well as minimisation of the prize $\Gamma$.




==> experimentsp2.tex <==
\begin{figure*}
\centering
\subfloat[Holes in conflicts]{
\scalebox{.23}{
\input{figures/dpmwhichholes.pgf}
}
\label{fig:whichholes}
}
\vspace{-1mm}
\caption{Performance graphs on DPM}
\label{fig:scalability}
\vspace{-2mm}
\end{figure*}




\subsection{Effect of properties and property thresholds}
In contrast to the baseline, the performance of our framework significantly depends on the properties forming the $\texttt{Unsat}$ specification. 
We first consider only $\Phi_1$. 
We vary the property thresholds from $0.7 \cdot \lambda^{*}$ to $0.95 \cdot \lambda^{*}$, where $\lambda^{*}$ is the optimal (i.e. minimal) value that can be achieved within the design space. 
The design space includes DTMCs having on average 5K relevant states, ranging from 2K to 8K~states. 

We observe a strong dependency between the performance (including the number of designs that has to be explored 
to prove that no valid realisation exists and the total runtime of the synthesis process) and the threshold. Fig.~\ref{fig:dpm2onlyqueue} shows the number of explored realisations (left axis, green circle) and the runtime in seconds (right axis, blue circle) for several thresholds. We obtain a speedup of a factor 100 over the baseline for the threshold of $0.7 \cdot \lambda^{*}$, that drops to factor 23 for the threshold  $0.95 \cdot \lambda^{*}$. Thus,  
\emph{the ``more unsatisfiable'' the synthesis problem is, the faster the framework is}. 

This correlation is mainly accounted for by the larger conflict sizes, i.e., less pruning. 
Consider the lines (queue-0.7) and (queue-0.95) in Fig.~\ref{fig:conflict_sizes}, that refer to these two different thresholds. 
The plot reports how often (y-axis, logscale) a conflict of a given size (x-axis) was found. 
We add lines to the histogram for better readability. 
Indeed, one can see that for (queue-0.7), the conflicts are always at most of size $7$, whereas for (queue-0.9) 200 trivial conflicts are found (size $9$). The more limited pruning is reflected by the number of designs explored (see Fig.~\ref{fig:dpm2onlyqueue}).
A second effect is that the average time per conflict analysis is also increased. 
The longer runtime originates from the optimistic approach of~\cite{Dehnert2014} and its search for the smallest CE. 
The net effect in the context of this framework is that conflict analysis becomes more costly but prunes less. 
%The conflict analysis procedure spends more time when pruning less.
In fact, for (queue-0.7), $85\%$ of the total time is spent in conflict analysis, for (queue-0.95) it is $93\%$.

To further demonstrate the critical impact of the conflict sizes, we consider $\Phi_2$.
 We vary the property thresholds from $0.7 \cdot \lambda^{*}$ to $0.9 \cdot \lambda^{*}$, where $\lambda^{*}$ is the optimum. 
%Fig.~\ref{fig:dpm2onlypower} shows the results. 
%The underlying DTMCs have slightly more relevant states, averaging around 6K~states.
Comparing to property $\Phi_1$ (Fig.~\ref{fig:dpm2onlyqueue}), we observe that 10 to 15 times more realisations are explored, which leads to a major slowdown. Consequently, the speedup versus the baseline drops to a factor of 2.5 and 1.1 for the threshold $0.7 \cdot \lambda^{*}$ and $0.9 \cdot \lambda^{*}$, respectively. 
To explain this drastic performance degradation, observe the conflict sizes for different properties and thresholds in Fig.~\ref{fig:conflict_sizes}. It is surprising that the framework still provides a (marginal) speedup although a very large number of trivial conflicts (of size 9) are found.

Finally, we explore the effect of a more complicated specification that includes multiple properties. 
In particular, we consider all three properties for the DPM model. We select thresholds ($7 \cdot \lambda^{*}$ for $\Phi_1$, $7 \cdot \lambda^{*} $ for $\Phi_3$, and $1.2 \cdot \lambda^{*}$ for $\Phi_2$)  that can be satisfied if considered alone, but not together. 

%\color{red} [ToDo Can we list the thresholds? -- $1.2 \cdot \lambda^{*}$ for energy, $2 \cdot \lambda^{*}$ for queues] \color{black}

As shown in Fig.~\ref{fig:conflict_sizes}, for the combined property, there are significantly fewer large conflicts (see line $\texttt{all}$). The graph indicates --- backed by close inspection of log files --- that realisations which allow only little pruning
for one property often provide a substantial pruning for the other property, especially if the two properties induce a trade-off as the energy consumption and the number of lost request representing reliability. 
Consequently, the speedup versus the baseline is about a factor 33,  which is better than the speedup of any of the properties considered independently.

Considering different specifications for the synthesis problem leads us to the conclusion that \emph{the properties have a crucial effect on the performance, however, having a richer specification with antagonistic properties significantly increases the potential of the CE-driven pruning}.  




%The combined property is evaluated quicker than for either property apart, even though the number of model checking queries is tripled, both internally and in the verification.
%The setup times do not need to be tripled, as in this special case --same path formulae in all properties -- we reuse information.
%We obtain a speedup of 33, which is better than the speedup of any of the properties considered independently.

%To review what happens, consider the all in Fig.~\ref{fig:conflict_sizes}. 
%Although counterexamples for these thresholds are harder to find than the two 'hard' lines, we see especially fewer %very large conflicts.
%The graph indicates -- backed by close inspection of log files -- that restrictions which allow only a bit of pruning by one property can often be pruned well via the other property, especially if the two properties induce a trade-off.


%If we optimise, [ I would tend to just put numbers in here, saying that we are slightly slower due a worse start. ]


\subsection{Effect of the size of the underlying DTMCs}
To evaluate the effect of the sizes of the instantiated DTMCs of a sketch, we use an unrolling of the DTMCs that allows us to increase their size without affecting the property satisfaction. 
Using a blow-up factor (B-UP), we increase the sizes of the particular DTMCs by about a factor of $2$ and $5$, respectively.

As shown in Fig.~\ref{fig:scalability} by the crosses and plusses in green (mostly overlapping), the number of designs explored is not significantly affected by larger state spaces. Slight deviations can be explained by the slightly different structure which leads to the discovery of other CEs. 
For both the baseline and the conflict analysis the runtimes grow linearly with the DTMC sizes, as long as the DTMCs easily fit into memory.
Larger models are less affected by the overhead of initialising the conflict analysis which leads to improved speedups on bigger models, especially for thresholds far  from the optimum.

%This claim is backed up by the timings of the components of the framework \color{red} [ToDo A short version of the commented text below + maybe a figure but I don't we need so detailed figure]


%The claims above are backed up by the timings of the components of the framework, given by the 4 pairs of bars in Fig.~\ref{fig:dpm2performance}. Timings are relative and the components sum to one.
%In each pair of bars, the left bar shows from bottom to top, timing for the SMT-solver (barely visible), the model-generation in the verifier, the counterexample generation, and the verification time.
%The right bar gives a break-down of the conflict analysis. 
%It contains, from bottom to top, set-up of the solver, the generation of the $\Upsilon$ (cuts), intermediate model checking, the (max)sat solver, and the evaluation of maxsat and model-checking results.
%The pairs of bars are of the form (threshold / blowup).
%Conflict analysis always takes most time.
%The relative time for the set-up diminishes as more and more candidates for counterexamples are generated, checked and evaluated.

%[the following is still to hard]
%Roughly, we see how, relatively, conflict analysis takes much more time for a threshold $0.9 \cdot \lambda^{*}$) than for the lower threshold.
%Likewise, we can compare to the bars for larger DTMCs, same threshold, on the right.
%While model checking gets more expensive, the single call isn't weighing in against the increased model building and conflict analysis time.
%We observe that model generation and conflict analysis both get relatively more expensive than model checking. 
%Within the conflict analysis, the maxsat solver mostly depends on the structure of the problem and the number of iterations, so that becomes relatively faster as evaluation, and especially model checking gets more expensive.


Based on these observations we conclude that \emph{the speedup achieved with respect to the baseline is not considerably affected by the size of the underlying DTMCs.} The influence of the properties and threshold is also preserved.


%\paragraph*{Variants}
%We consider one of the other properties, the expected energy consumption, in Fig.~\ref{fig:dpm2onlypower}. 
%The relevant model averages --without blow-up-- at 6000 states (ranging from 2000 to 10000).
%This property allows for less pruning. 
%For a threshold $\sim 0.9 \cdot \lambda^{*}$, the speed up is only $12\%$.
%%The blown-up version is roughly $50\%$ larger, as are the runtimes.
%Fig.~\ref{fig:conflict_sizes} shows that 
%Considering the extreme amount of trivial conflicts, it is interesting that the framework still obtains a (marginal) speed up. 

%After we have considered these two properties apart, we consider looking for a sketch that satisfies three properties. 
%The queue occupancy (for both queues, the properties are symmetric), and the expected energy consumption. 
%We select thresholds for the properties that can be satisfied if considered alone.
%The combined property is evaluated quicker than for either property apart, even though the number of model checking queries is tripled, both internally and in the verification.
%The setup times do not need to be tripled, as in this special case --same path formulae in all properties -- we reuse information.
%We obtain a speedup of 33, which is better than the speedup of any of the properties considered independently.

%To review what happens, consider the all in Fig.~\ref{fig:conflict_sizes}. 
%Although counterexamples for these thresholds are harder to find than the two 'hard' lines, we see especially fewer %very large conflicts.
%The graph indicates -- backed by close inspection of log files -- that restrictions which allow only a bit of pruning by one property can often be pruned well via the other property, especially if the two properties induce a trade-off.


%If we optimise, [ I would tend to just put numbers in here, saying that we are slightly slower due a worse start. ]


\subsection{Effect of the sketch structure}
\label{sec:sketcheffect}

To understand how the performance is affected by the structure of the sketch,
 we evaluate the effect of the particular holes (recall: there are 9 holes). 
 Fig.~\ref{fig:whichholes} presents how often (x-axis) the holes are included in a conflict (the orange bar is for $\Phi_1$ with threshold $0.7 \cdot \lambda^{*}$, the blue bar is for $\Phi_2$ with threshold $0.4 \cdot \lambda^{*}$ and also goes from 0). 
The selected thresholds are not important for the message:
How often a hole appears varies wildly.
Roughly, the higher the bar the harder it is to prune options in that hole. 
The hardness of a hole is (informally) correlated to the probability mass of relevant paths touching commands containing the hole. 
More precisely, the hardness is partially affected by the DTMC topology --- hole X11 is in the command that is enabled in the initial state and thus, it is touched by all probability mass, and always in the conflict --- and partially as a consequence of the property --- for $\Phi_2$, holes X13 and X31 are equally hard as the paths through them are equally relevant for the property $\Phi_2$, but not for $\Phi_1$. 
To improve understanding, we review the properties on some adapted design spaces.

The plot in Fig.~\ref{fig:dpm2variants} is similar as Fig.~\ref{fig:dpm2onlyqueue} (it shows the results for property  $\Phi_1$ with threshold $0.7 \cdot \lambda^{*}$), however, on the X-axis we now have four different design spaces: 
In V1 and V2, we instantiate hole X11 with an option beneficial for satisfying the property, and a disadvantageous option respectively, as we do in V3 and V4 for hole X33.
All obtained design spaces are equally large and the baseline takes equally long for all of them.
Recall that for the original (with B-UP=5), the speedup is a factor 23.
The variants (with B-UP=5) have speedups between a factor 40 (for V3) and 550 (for V2). Thus, all variants profit from the reduced number of relevant commands, by a decreased runtime of more than a factor 4 (= reduction of the design space).
Note that V1, V3 profit less than V2, V4 from the hole instantiation because V2 and V4 are ``farther away from satisfiability.'' Also note that instantiating holes that are less hard might be disadvantageous for the obtained speedup.

The massive performance gain for V2 is explained by the fact that the instantiated hole X11 is always enabled, so it was part of every conflict. Consequently, all conflicts were at least one larger than in variant V2. 
This strong reduction in the conflict sizes does not hold for V4, because it still contains X11 as a hole, and X33 was not always part of a conflict. Finally, consider the holes X31 and X13 (with the low bars) in the original sketch. These holes are very suitable for pruning and thus the framework is able to efficiently prune disadvantageous options added to the sketch 
without affecting the runtime much. We summarize these observations as follows:

\emph{The framework performs better (by orders of magnitude) on sketches with holes that do not lie on many relevant paths. Extending such holes with clearly inferior options hardly affects to runtime, as these options will be pruned efficiently. }

%I would drop this.
%[This is about the original sketch. Should we discuss it? -- I would ]
%%The sketch considered has holes in a one-to-one correspondence to grids.
%If we vary the sketch such that now also the areas are described by holes, then these holes occur in several commands. 
%However, in our example with a design space of 30000, we still had a slight speedup, as the number of relevant commands was only 5 (yielding a maximum of $2^5=32$ model checking invocations per conflict analysis, rather than the $2^9=512$ in the original sketch).


 
 


%
%Results for satisfiable designs were consequently strongest affected by the random seed, which makes a fair comparison difficult. 
%However, lessons above mostly carry over, with the following adaption:
%The more satisfiable, the more likely it is to accidentally hit a satisfiable instance, which makes the effect of pruning eventually diminish for designs where every realisation is satisfying.
%Pruning is helpful, if it is applied to harder instances.  
%Thorough development and evaluation of heuristics that quickly find a satisfying realisation is left for future work.\footnote{As heuristics that over-fit to the characterisations of sketch were, given the unavailability of a large corpus of sketches, simple to develop and generally work well.}
%%
%Conclusions:
%\begin{itemize}
%\item An important observation of single counterexample generation in \cite{} is that naturally, the closer the actual performance is to the desired performance, the more every part of the model adds, and the bigger the counterexamples. This observation carries over to generalisation: 
% \item Conflict-analysis is especially well-suited to prevent repetitive analysis with (very) poor options. Put differently, \emph{the better the sketch, the less significant is the help}.
% \item 
%\end{itemize}
%
%
%\subsection{Method evaluation}

\subsection{Validating results on other scenarios}

%Beyond improved performance, we argue that the counterexample driven analysis offers additional benefits. 
%\begin{itemize}
%\item What insights beyond "computers says no" does the framework deliver upon reporting unsatisfiability. (and computer says yes)?
%\end{itemize}
%
%\emph{Conclusions drawn from the absence of conflicts} have to be treated carefully. The absence can be due to two orthogonal effects: 
%First, the absence might be hidden, as instances in which a counterexample would occur are never explored. This problem might be overcome by exploring all instances, thereby ignoring the original idea of pruning the instances that are explored.
%Second, the absence might be due to notion of a highlevel counterexample as the conflict.
%We illustrate these two shortcomings:
%
%
%\subsection{Pruning}
%
%In the naive setting, each model is constructed once, and model checked at most $|\varphi|$ times.
%
%What affects the size of the pruning:
%
%


\color{black}
The intrusion scenario has 26 holes and a design space of 6800K realisations.% (that satisfy the constraints).
The average size of the underlying DTMCs is 500 states.
Comparing to the DPM model, we observe an even more significant effect of the property thresholds on the performance. With respect to the baseline, we obtain a speedup of factor $2200$, $250$ and $5$, for thresholds $0.7 \cdot \lambda^{*}$, $0.8 \cdot \lambda^{*}$ and $0.9 \cdot \lambda^{*}$, respectively. With the larger sets of relevant commands, moving closer to the optimum is more expensive (recall that we use an optimistic verifier). 
Conversely, for less strict thresholds, pruning is even more effective with many conflicts containing only 8 out of 26 holes. 
Scaling the model size again does not affect the obtained speedups.
We also varied the design space by instantiating holes as in Sect.~\ref{sec:sketcheffect}. 
The performance differences among the considered variants is much alike Fig.~\ref{fig:dpm2variants}, and the differences can be explained via the hardness of the holes.
In contrast to the DPM variants, the overall speedups remain closer to the original sketch.

For the grid scenario, we present results for a structurally different synthesis problem including 
small design space with 6 holes (in the 3 commands) and 1800 realisations. The average size of the underlying DTMC is, however, 100K states. Not all realisations ensure that we almost surely reach the target (which is implied by the specification). We therefore (automatically) add a lower-bounded property ensuring that we reach the target with probability 1, and apply the conflict analysis technique discussed in Sect.~\ref{sec:algorithmic:extendedmaxsat}. %For these realisations, the obtained counterexample were typically still minimal, despite the lack of a formal guarantee.
Due to the topology of the DTMCs and as each relevant command contains two holes, holes are very hard (recall the discussion in Sect.~\ref{sec:sketcheffect}): More than 70\% of the conflicts are trivial, and 25\% of the designs are explored. Still, we obtain a speedup a factor 3 for the threshold $0.98 \cdot \lambda^{*}$. In contrast to the previous case studies, the speedup is not significantly affected by the thresholds due to the qualitative nature of the ${\geq 1}$ threshold of the additional property. 

